Axiomatic Preference Modeling for Longform Question Answering

The remarkable abilities of large language models (LLMs) like GPT-4 partially stem from post-training processes like Reinforcement Learning from Human Feedback (RLHF) involving human preferences encoded in a reward model. However, these reward models (RMs) often lack direct knowledge of why, or under what principles, the preferences annotations were made. In this study, we identify principles that guide RMs to better align with human preferences, and then develop an axiomatic framework to generate a rich variety of preference signals to uphold them. We use these axiomatic signals to train a model for scoring answers to longform questions. Our approach yields a Preference Model with only about 220M parameters that agrees with gold human-annotated preference labels more often than GPT-4. The contributions of this work include: training a standalone preference model that can score human- and LLM-generated answers on the same scale; developing an axiomatic framework for generating training data pairs tailored to certain principles; and showing that a small amount of axiomatic signals can help small models outperform GPT-4 in preference scoring. We release our model on huggingface: https://huggingface.co/corbyrosset/axiomatic_preference_model

==> tables/hard_neg_answer_reranking_results.tex <==
% \begin{wrapfigure}{r}{0.5\textwidth}
% \begin{minipage}{0.5\textwidth}
\begin{table}
\centering
\begin{tabular}{l|lll}
\cline{2-4}
       & \multicolumn{3}{c|}{StackX human answers only}                         \\
Model  & \multicolumn{1}{c}{MRR (top)} & MRR (any) & \multicolumn{1}{l|}{NDCG} \\ \hline
random & -                             &           &                           \\
length &                               &           &                           \\ \hline
ChatGPT pointwise   &                               &           &                           \\
\multicolumn{1}{r|}{+ guidelines}   &                               &           &                           \\
GPT-4 listwise & & & \\
\hline 
\preferencemodel Axiom0 &                               &           & \\
+ Axiom 1 &                               &           & 
\end{tabular}
\label{tab:answer-reranking-hardneg}
\captionof{table}{Using the \preferencemodel to re-rank set of \{human answers\} $\cup$ \{hard negatives\} for each question. Hard negative mining retrieved about 40 additional answers to topically related questions}
\end{table}
% \end{minipage}
% \end{wrapfigure}



==> tables/rank_of_LLM_answers.tex <==
\begin{table} %{0.5\textwidth}
\centering
\begin{tabular}{l|ll}
\cline{2-3}
       & \multicolumn{2}{c|}{StackXChange}                         \\
Model  & \multicolumn{1}{c}{MRR (ChatGPT)} & \multicolumn{1}{l|}{MRR (GPT-4)} \\ \hline
random & -  &  \\
GPT-4 & & \\
\hline 
\preferencemodel Axiom0 &                               &           \\
+ Axiom 1 &                               &           
\end{tabular}
\label{tab:rank-of-llm-answers}
\captionof{table}{Using various \preferencemodel to rank how highly a closed-book ChatGPT or GPT-4 answer is among the human-written answers for each question}
\end{table}


